Collaborative Expert LLMs Guided Multi-Objective Molecular Optimization

Molecular optimization is a crucial yet complex and time-intensive process that often acts as a bottleneck for drug development. Traditional methods rely heavily on trial and error, making multi-objective optimization both time-consuming and resource-intensive. Current AI-based methods have shown limited success in handling multi-objective optimization tasks, hampering their practical utilization. To address this challenge, we present MultiMol, a collaborative large language model (LLM) system designed to guide multi-objective molecular optimization. MultiMol comprises two agents, including a data-driven worker agent and a literature-guided research agent. The data-driven worker agent is a large language model being fine-tuned to learn how to generate optimized molecules considering multiple objectives, while the literature-guided research agent is responsible for searching task-related literature to find useful prior knowledge that facilitates identifying the most promising optimized candidates. In evaluations across six multi-objective optimization tasks, MultiMol significantly outperforms existing methods, achieving a 82.30% success rate, in sharp contrast to the 27.50% success rate of current strongest methods. To further validate its practical impact, we tested MultiMol on two real-world challenges. First, we enhanced the selectivity of Xanthine Amine Congener (XAC), a promiscuous ligand that binds both A1R and A2AR, successfully biasing it towards A1R. Second, we improved the bioavailability of Saquinavir, an HIV-1 protease inhibitor with known bioavailability limitations. Overall, these results indicate that MultiMol represents a highly promising approach for multi-objective molecular optimization, holding great potential to accelerate the drug development process and contribute to the advancement of pharmaceutical research.

==> support_information.tex <==
\section{Support Information}
\begin{table}[h!]
\centering
\caption{Task Performance Metrics for Single and Multi-Property Optimization on Unseen Smiles }
\begin{tabular}{lcccc}
\toprule
\textbf{Task ID} & \textbf{Hit Ratio (Loose)} & \textbf{Hit Ratio (Strict)} & \textbf{Valid Ratio} & \textbf{Same Scaffold Ratio} \\
\midrule
\multicolumn{5}{c}{\textit{Single Property Optimization}} \\
\midrule
101 & 97.32 & 94.39 & 98.13 & 79.27 \\
102 & 93.19 & 85.64 & 99.36 & 89.29 \\
103 & 52.52 & 20.62 & 97.71 & 93.77 \\
104 & 88.86 & 67.80 & 98.81 & 86.92 \\
105 & 64.82 & 55.42 & 98.26 & 90.84 \\
106 & 99.04 & 98.56 & 98.93 & 83.73 \\
107 & 99.02 & 97.07 & 98.13 & 82.44 \\
108 & 95.10 & 89.71 & 98.69 & 84.31 \\
\midrule
\multicolumn{5}{c}{\textit{Multiple Properties Optimization}} \\
\midrule
201 & 92.77 & 87.71 & 99.26 & 81.93 \\
202 & 49.86 & 23.77 & 97.53 & 87.25 \\
203 & 91.97 & 83.70 & 98.36 & 81.27 \\
204 & 38.66 & 10.64 & 99.22 & 80.67 \\
205 & 32.29 & 19.76 & 97.25 & 88.67 \\
206 & 91.08 & 82.41 & 98.26 & 85.30 \\
\bottomrule
\end{tabular}
\label{tab_leakage}
\end{table}

\paragraph{Analysis of data leakage}
To investigate whether the impressive performance of MultiMol is attributable to prior exposure to small molecules, we aimed to address potential data leakage issues. To this end, we utilized new molecules sourced from Public Access to Neuroactive Anticonvulsant Chemical Evaluations (PANAChE) \footnote{\url{http://panache.ninds.nih.gov} }, published on October 24, 2024, which were specifically designed for screening neurological diseases and strokes.
The performance metrics for both single and multi-property optimization tasks on these unseen SMILES representations are presented in Table \ref{tab_leakage}. Our analysis reveals that Galactica continues to exhibit strong performance metrics across various tasks. For instance, in single property optimization, the hit ratios (both loose and strict) consistently exceed 50\%, with several tasks achieving impressive hit ratios above 90\%. Notably, Task ID 106 stands out with a loose hit ratio of 99.04\% and a strict hit ratio of 98.56\%, indicating robust model performance even on unseen data.
Similarly, the multi-property optimization tasks yield comparable results, with Task ID 201 achieving a hit ratio of 92.77\% (loose) and 87.71\% (strict). Although some tasks, such as Task ID 204, show lower hit ratios, the valid and same scaffold ratios remain relatively high, suggesting that the model is capable of generating relevant molecular structures while adhering to input scaffold constraints.
Overall, these findings suggest that MultiMol's performance is resilient, even when tested with novel molecules, reinforcing the validity of its predictive capabilities in molecular optimization tasks without evidence of data leakage. This further highlights the model's potential utility in drug discovery and molecular design.





\begin{table}[ht]
    \centering
    \caption{Performance metrics for various backbones and task IDs.}
    \begin{tabular}{lcccccc}
        \toprule
        Backbone & Task ID & Hit Ratio (Loose) & Hit Ratio (Strict) & Valid Ratio & Same Scaffold Ratio \\
        \midrule
\multicolumn{6}{c}{\textit{Single Property Optimization}} \\
\midrule
        qwen2.5-7b & 101 & 74.09 & 46.63 & 96.50 & 90.67 \\
        qwen2.5-7b & 102 & 29.84 & 14.66 & 95.50 & 87.43 \\
        qwen2.5-7b & 103 & 58.03 & 17.10 & 96.50 & 94.30 \\
        qwen2.5-7b & 104 & 39.90 & 13.47 & 96.50 & 93.78 \\
        qwen2.5-7b & 105 & 57.59 & 44.50 & 95.50 & 93.19 \\
        qwen2.5-7b & 106 & 15.43 & 8.51 & 94.00 & 87.77 \\
        qwen2.5-7b & 107 & 4.21 & 2.63 & 95.00 & 91.05 \\
        qwen2.5-7b & 108 & 19.79 & 5.73 & 96.00 & 91.67 \\
        llama3.1-8b & 101 & 75.00 & 50.00 & 16.00 & 75.00 \\
        llama3.1-8b & 102 & 21.62 & 18.92 & 18.50 & 75.68 \\
        llama3.1-8b & 103 & 45.16 & 12.90 & 15.50 & 90.32 \\
        llama3.1-8b & 104 & 55.17 & 31.03 & 14.50 & 75.86 \\
        llama3.1-8b & 105 & 57.97 & 44.93 & 34.50 & 81.16 \\
        llama3.1-8b & 106 & 33.33 & 22.22 & 18.00 & 80.56 \\
        llama3.1-8b & 107 & 23.53 & 23.53 & 17.00 & 79.41 \\
        llama3.1-8b & 108 & 23.08 & 7.69 & 19.50 & 69.23 \\
        \midrule
\multicolumn{6}{c}{\textit{Multiple Properties Optimization}} \\
\midrule
        qwen2.5-7b & 201 & 2.34 & 0.58 & 85.50 & 72.51 \\
        qwen2.5-7b & 202 & 7.83 & 3.01 & 83.00 & 65.66 \\
        qwen2.5-7b & 203 & 16.57 & 4.42 & 90.50 & 77.35 \\
        qwen2.5-7b & 204 & 6.59 & 3.30 & 91.00 & 73.08 \\
        qwen2.5-7b & 205 & 40.32 & 14.52 & 93.00 & 82.80 \\
        qwen2.5-7b & 206 & 12.43 & 6.21 & 88.50 & 68.93 \\
        llama3.1-8b & 201 & 23.40 & 17.02 & 23.50 & 74.47 \\
        llama3.1-8b & 202 & 14.04 & 10.53 & 28.50 & 73.68 \\
        llama3.1-8b & 203 & 45.95 & 24.32 & 18.50 & 72.97 \\
        llama3.1-8b & 204 & 18.60 & 13.95 & 21.50 & 60.47 \\
        llama3.1-8b & 205 & 37.84 & 24.32 & 37.00 & 72.97 \\
        llama3.1-8b & 206 & 36.21 & 24.14 & 29.00 & 75.86 \\
        \bottomrule
    \end{tabular}
    \label{tab_backbone}
\end{table}


\paragraph{Analysis of backbone}
To explore whether other large language models (LLMs) can achieve satisfactory results in molecular optimization tasks, we conducted fine-tuning experiments on other mainstream LLM architectures as shown in Table \ref{tab_backbones}. Specifically, we chose llama3.1 and qwen2.5 as our subjects and employed the following prompt for fine-tuning: \textit{Please recover this masked molecule [SCAFFOLD], the desired properties is [SOURCE PROPERTY]. The recover molecule is [SOURCE MOLECULE].} The models were fine-tuned with identical parameters.

In our experiments across 14 optimization tasks, we found that, overall, both backbones performed worse than galactica6.7b, exhibiting lower hit ratios. Moreover, llama3.1-8b also demonstrated a lower valid ratio, suggesting that these general-purpose language models may have too broad a knowledge base, hindering their ability to generate more accurate molecules. However, it is noteworthy that both models maintained a respectable same scaffold ratio, indicating that this scaffold-based fine-tuning strategy more effectively encourages LLMs to generate molecules similar to the input scaffolds. This finding provides critical insights for future research, emphasizing the importance of model architecture and fine-tuning strategies in molecular generation tasks.




\paragraph{Analysis of recovering molecules}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/regression_combined.pdf}
    \caption{\textbf{MultiMol Recovery Performance.} Density plots illustrating the ability of MultiMol to recover the original molecules using the prompt $(Source\ Property + Scaffold) \rightarrow Source\ Molecule$. Each subfigure shows the distribution of specific molecular properties (MolLogP, QED, TPSA, NumHAcceptors, and NumHDonors) for both the source and recovered molecules, with the mean values indicated by dashed lines.}
    \label{fig_recover}
\end{figure}


As shown in Figure \ref{fig_recover}, the distributions of LogP, QED, TPSA, \#HAcceptors, and \# HDonors exhibit strong alignment between source (green) and recovered (purple) properties, with closely matched peaks and nearly overlapping mean values (dashed lines). This indicates effective retention of these molecular properties during recovery.
For QED, the source and recovered distributions align closely, with only minimal variation at the distribution tails, demonstrating strong fidelity in preserving drug-likeness. Similarly, TPSA shows a consistent pattern, with the recovered values slightly shifted, reflecting subtle adjustments in polar surface area.
Overall, these results demonstrate that the recovery process maintains most key molecular properties.


\subsection{Filter rules}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/rules_single.pdf}
    \caption{Impact of candidate molecule pool size on single-property optimization metrics. For a pool size of 1, the model operates without rule-based filtering. Each panel illustrates the distribution of a specific molecular property (MolLogP, QED, TPSA, NumHAcceptors, and NumHDonors) across different pool sizes.}
    \label{fig_rules}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/rules_multi.pdf}
    \caption{Impact of candidate molecule pool size on multi-property optimization metrics. With a pool size of 1, the model operates without rule-based filtering. Each panel shows the distribution of various molecular properties (MolLogP, QED, TPSA, NumHAcceptors, and NumHDonors) across different pool sizes.}
    \label{fig_rules}
\end{figure}

\paragraph{Analysis of rules}
This figure \ref{fig_rules} represents the performance of the proposed DAMO framework across multiple molecule optimization tasks (Task 101 to Task 108). Each subfigure illustrates the impact of the number of generated molecules on four key metrics: Hit Ratio (Loose), Hit Ratio (Strict), Valid Ratio, and Same Scaffold Ratio. These metrics are plotted against the number of generated molecules, with the x-axis using a logarithmic scale to indicate the progressive increase in the number of the generated molecules.
The hit ratio (loose, in pink) and hit ratio (strict, in orange) improve consistently as more molecules are generated across all tasks. For tasks such as 106 and 107, the loose hit ratio sees a particularly steep increase, indicating the method's ability to improve hit rates with larger molecule sets. However, the strict hit ratio (which imposes stricter criteria) starts lower across all tasks but also improves as the number of molecules increases.
Across all tasks, the valid ratio (green) remains nearly constant at 100\%, suggesting that the majority of the generated molecules are chemically valid. This result is expected, as ensuring molecule validity is crucial in drug discovery.
Same Scaffold Ratio: The same scaffold ratio (brown) shows a varied pattern. In some tasks, like Task 106 and Task 104, this ratio increases significantly with more generated molecules, suggesting that scaffold consistency improves with more data. However, in other tasks such as Task 103 and Task 108, the scaffold ratio stays relatively flat, indicating that scaffold consistency may not be as easily maintained depending on the task.
The framework performs differently across tasks, as seen in the variations in the strict hit ratio and scaffold consistency. This suggests that the efficacy of the DAMO framework may depend on the specific properties of the dataset and the molecule classes involved in each task.
Tasks 104 and 106 display the highest improvement in the same scaffold ratio as more molecules are generated, implying that these tasks might benefit more from scaffold-specific fine-tuning and prior knowledge integration. However, tasks like 103 show a clear trade-off where improving scaffold consistency may be more challenging.
\textbf{Scalability of Molecule Generation}: The steady improvement in hit ratios as more molecules are generated highlights the DAMO framework's scalability. This shows that the model benefits from increased data, supporting the use of large-scale molecule generation to achieve better optimization results.
The figure effectively demonstrates the DAMO framework's capability to optimize molecules across different tasks, with a consistent improvement in hit ratios and a generally stable valid ratio. The variability in scaffold consistency across tasks underscores the challenge of maintaining scaffold integrity, which the framework attempts to address. These results emphasize the model's robustness in generating valid molecules, though scaffold consistency may require further refinement in some cases. Overall, the figure supports the claim that DAMO leverages both data-driven and prior knowledge-driven approaches to achieve better molecule optimization outcomes.


% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{fig/multi-scatter.pdf}
%     \caption{Scatter plots illustrating the distribution of source (blue) and generated (purple) molecules across multiple tasks (201 to 206) for multi-property optimization. Each subplot represents a specific task, with individual points showing samples of molecules and stars indicating the central points of the source and generated molecule distributions. Arrows connect the centers of the source and generated molecule clusters, highlighting shifts in property distributions as a result of optimization.}
%     \label{fig_rules}
% \end{figure}


\begin{table}[h!]
    \centering
    \renewcommand{\arraystretch}{1.5} % Increase row height for better readability
    \begin{tabular}{|>{\centering\arraybackslash}m{6cm}|>{\centering\arraybackslash}m{11cm}|}
        \hline
        \textbf{Task Description} & \textbf{Prompt Template} \\
        \hline
        \textbf{GALACTICA Small Molecule Fine-Tuning} & 
        \texttt{<s> Masked SMILES: [START\_SMILES] \{ \} [END\_SMILES], properties: \{ \}. Completed SMILES: [START\_SMILES] \{ \} [END\_SMILES]. </s>} \\
        \hline
        \textbf{Other LLM Fine-Tuning} & 
        \texttt{Please recover this masked molecule \{ \}, the desired properties are \{ \}. The recovered molecule is \{ \}} \\
        \hline
        \textbf{GALACTICA Molecule-Protein Fine-Tuning} & 
        \texttt{<s> Masked SMILES: [START\_SMILES] \{ \} [END\_SMILES], property: \{ \}, the affinity between the molecule and the protein [START\_AMINO] \{ \} [END\_AMINO] is \{ \}. Completed SMILES: [START\_SMILES] \{ \} [END\_SMILES]. </s>} \\
        \hline
        \textbf{GALACTICA Small Molecule Inference} & 
        \texttt{<s> Masked molecule [START\_SMILES] \{ \}[END\_SMILES], property: \{ \}. Completed molecule: [START\_SMILES]} \\
        \hline
        \textbf{Other LLM Inference} & 
        \texttt{Please recover this masked molecule \{ \}, the desired properties are \{ \}. The recovered molecule is} \\
        \hline
        \textbf{GALACTICA Molecule-Protein Inference} & 
        \texttt{<s> Masked SMILES: [START\_SMILES] \{ \} [END\_SMILES], property: \{ \}, the affinity between the molecule and the protein [START\_AMINO] \{ \} [END\_AMINO] is \{ \}. Completed SMILES: [START\_SMILES] \{ \} [END\_SMILES]} \\
        \hline
    \end{tabular}
    \caption{Prompt Templates for Fine-Tuning and Inference on Molecule and Protein Tasks}
\end{table}



